Analytic Performance Model of a Main-Memory Index Structure

Efficient evaluation of multi-dimensional range queries in a main-memory database is an important, but difficult task. State-of-the-art techniques rely on optimised sequential scans or tree-based structures. For range queries with small result sets, sequential scans exhibit poor asymptotic performance. Also, as the dimensionality of the data set increases, the performance of tree-based structures degenerates due to the curse of dimensionality. Recent literature proposed the Elf, a main-memory structure that is optimised for the case of such multi-dimensional low-selectivity queries. The Elf outperforms other state-of-the-art methods in manually tuned scenarios. However, choosing an optimal parameter configuration for the Elf is vital, since for poor configurations, the search performance degrades rapidly. Consequently, further knowledge about the behaviour of the Elf in different configurations is required to achieve robust performance. In this thesis, we therefore propose a numerical cost model for the Elf. Like all main-memory index structures, the Elf response time is not dominated by disk accesses, refusing a straightforward analysis. Our model predicts the size and shape of the Elf region that is examined during search. We propose that the response time of a search is linear to the size of this region. Furthermore, we study the impact of skewed data distributions and correlations on the shape of the Elf. We find that they lead to behaviour that is accurately describable through simple reductions in attribute cardinality. Our experimental results indicate that for data sets of up to 15 dimensions, our cost model predicts the size of the examined Elf region with relative errors below 5%. Furthermore, we find that the size of the Elf region examined during search predicts the response time with an accuracy of 80%.

==> real_source_texlive_2016/sections/abstract_de.tex <==
\Abstract
Die effiziente Auswertung von mehrdimensionalen Bereichsanfragen ist eine wichtige
Aufgabe für hauptspeicherbasierte Datenbanksysteme.
Aktuelle Ansätze
verwenden optimierte lineare Suchen oder baum-basierte Indexstrukturen zur Beantwortung solcher Anfragen.
Für Anfragen mit verhältnismäßig wenigen Ergebnissen verlieren
lineare Suchen jedoch aufgrund der linearen asymptotischen Komplexität an Leistung.
Weiterhin wirkt bei einer steigenden Anzahl von Attributen der Fluch der hohen Dimensionen
und die Suchgeschwindigkeit von Baumstrukturen sinkt.
Neueste Arbeiten führten den \say{Elf} ein, eine Datenstruktur
für Hauptspeicherindizes,
die für den Fall von mehrdimensionalen Anfragen mit kleiner Ergebnismenge optimiert ist.
Der Elf ist für diesen Anfragetyp potentiell schneller als andere bekannte Methoden.
Allerdings müssen dafür einige Parameter, wie die Reihenfolge der Attribute, optimal festgelegt werden.
Andernfalls sinkt die Suchgeschwindigkeit stark und der Elf wird unbrauchbar.
Dies führt zum Wunsch nach genauerem Wissen über das Verhalten des Elfen
in verschiedenen Parameterkonfigurationen.
In dieser Arbeit stellen wir deshalb ein numerisches Kostenmodell für den Elfen vor,
das die Ausführungszeit der Anfragenbearbeitung prognostiziert.
Problematisch ist dabei, dass der Elf eine Hauptspeicher-Indexstruktur ist;
derartige Strukturen sind normalerweise nicht einfach zu analysieren,
da der durch langsame Festplatten verursachte Flaschenhals wegfällt.
Unser Modell schätzt die Form und Größe des Elfen ab.
Dabei ist insbesondere der Teil der Struktur interessant,
der während der Bearbeitung einer Anfrage durch das Datenbanksystem betrachtet wird.
Darüber hinaus beschreiben wir, wie sich nicht gleichverteilte Daten und Korrelationen
auf die Struktur des Elfen auswirken.
Dabei stellen wir fest, dass diese Faktoren zu Verhaltensänderungen führen,
die durch einfache Veränderungen der Attributkardinalitäten akkurat modellierbar sind.
Die Ergebnisse unser empirischen Auswertung zeigen,
dass das Modell für Datensätze mit bis zu \num{15} Dimensionen die
Größe des Elfen mit relativen Fehlern unter \SI{5}{\percent} vorhersagt.
Weiterhin stellen wir fest, dass die Größe des Elfen die Ausführungszeit zu mehr als
\SI{80}{\percent} bestimmt.


==> real_source_texlive_2016/sections/abstract_en.tex <==
\Abstract
Efficient evaluation of multi-dimensional range queries in a main-memory database is an
important, but difficult task.
State-of-the-art techniques rely on optimised sequential scans or tree-based structures.
For range queries with small result sets, sequential scans exhibit poor asymptotic performance.
Also, as the dimensionality of the data set increases,
the performance of tree-based structures degenerates due to the curse of dimensionality.
%
Recent literature proposed the Elf, a main-memory structure that is
optimised for the case of such multi-dimensional low-selectivity queries.
The Elf outperforms other state-of-the-art methods in manually tuned scenarios.
However, choosing an optimal parameter configuration for the Elf is vital,
since for poor configurations, the search performance degrades rapidly.
%
Consequently, further knowledge about the behaviour of the Elf
in different configurations is required to achieve robust performance.
%
In this thesis, we therefore propose a numerical cost model for the Elf.
Like all main-memory index structures, the Elf
response time is not dominated by disk accesses, refusing a straightforward analysis.
Our model predicts the size and shape of the Elf region that is examined during search.
We propose that the response time of a search is linear to the size of this region.
Furthermore, we study the impact of skewed data distributions and correlations on the shape of the Elf.
We find that they lead to behaviour that is accurately describable through
simple reductions in attribute cardinality.
%
Our experimental results indicate that for data sets of up to \num{15} dimensions,
our cost model predicts the size of the examined Elf region with
relative errors below \SI{5}{\percent}.
Furthermore, we find that the size of the Elf region examined during search
predicts the response time with an accuracy of \SI{80}{\percent}.

